Skeleton Abstraction for Universal Temporal Properties

Uniform coloured Petri nets can be abstracted to their skeleton, the place/transition net that simply turns the coloured tokens into black tokens. A coloured net and its skeleton are related by a net morphism. For the application of the skeleton as an abstraction method in the model checking process, we need to establish a simulation relation between the state spaces of the two nets. Then, universal temporal properties (properties of the $ ACTL^* $ logic) are preserved. The abstraction relation induced by a net morphism is not necessarily a simulation relation, due to a subtle issue related to deadlocks. We discuss several situations where the abstraction relation induced by a net morphism is as well a simulation relation, thus preserving $ACTL^*$ properties. We further propose a partition refinement algorithm for folding a place/transition net into a coloured net. This way, skeleton abstraction becomes available for models given as place/transition nets. Experiments demonstrate the capabilities of the proposed technology. Using skeleton abstraction, we are capable of solving problems that have not been solved before in the Model Checking Contest.

==> pakete.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{geometry}
\usepackage{fancyhdr}
\usepackage{amsfonts}
\usepackage{times}
\usepackage{subcaption}
\usepackage{todonotes}

\usepackage{tikz}
\usetikzlibrary{arrows,shapes,snakes,automata,backgrounds,petri,positioning}
\tikzset{>=latex}

\usepackage{graphicx}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\newcommand\rot[1]{\textcolor{red}{#1}}

\usepackage{scalerel}
\newcommand{\N}{\scaleto{N}{3.2pt}}
\newcommand{\C}{\scaleto{C}{3.2pt}}
\newcommand{\U}{\scaleto{U}{3.2pt}}
\renewcommand{\S}{\scaleto{S}{3.2pt}}
\newcommand{\Sp}{\scaleto{S'}{3.2pt}}
\newcommand{\1}{\scaleto{1}{3.2pt}}
\newcommand{\2}{\scaleto{2}{3.2pt}}
\newcommand{\3}{\scaleto{2}{3.2pt}}

\renewcommand{\phi}{\varphi}
\newcommand\Tau{\mathcal{T}}
\newcommand\Kappa{\mathcal{C}}
\newcommand{\gdw}{\Leftrightarrow}
\newcommand\abs[1]{\vert #1 \vert}
\newcommand{\pre}[1]{\bullet #1}
\newcommand{\post}[1]{#1 \bullet}

\newcommand{\scopen}[1]{#1 \in \{1,\dots,n\}}
\newcommand{\scopek}[1]{#1 \in \{1,\dots,k\}}
\newcommand{\scopem}[1]{#1 \in \{1,\dots,m\}}

